DetectBERT: Towards Full App-Level Representation Learning to Detect Android Malware

Recent advancements in ML and DL have significantly improved Android malware detection, yet many methodologies still rely on basic static analysis, bytecode, or function call graphs that often fail to capture complex malicious behaviors. DexBERT, a pre-trained BERT-like model tailored for Android representation learning, enriches class-level representations by analyzing Smali code extracted from APKs. However, its functionality is constrained by its inability to process multiple Smali classes simultaneously. This paper introduces DetectBERT, which integrates correlated Multiple Instance Learning (c-MIL) with DexBERT to handle the high dimensionality and variability of Android malware, enabling effective app-level detection. By treating class-level features as instances within MIL bags, DetectBERT aggregates these into a comprehensive app-level representation. Our evaluation demonstrates that DetectBERT not only surpasses existing state-of-the-art detection methods but also adapts to evolving malware threats. Moreover, the versatility of the DetectBERT framework holds promising potential for broader applications in app-level analysis and other software engineering tasks, offering new avenues for research and development.

==> sections/RelatedWork.tex <==
\section{Related Work}
% Traditional malware detection approaches often struggle to keep pace with the rapid development of new and complex malware types~\cite{qiu2020survey,chowdhury2023android}.
% Recent advancements in machine learning~\cite{arp2014drebin,wu2019malscan} and deep learning~\cite{hsien2018r2,ding2020android,daoudi2021dexray} have offered promising avenues for enhancing Android malware detection. 
% However, the application of these advanced technologies to Android malware detection faces significant obstacles, as they largely depend on static analysis~\cite{fereidooni2016anastasia,sandeep2019static,pan2020systematic}, extracting basic features or low-level bytecode from APK files~\cite{daoudi2021dexray,sun2021android}, and analyzing function call graphs~\cite{pektacs2020deep,yang2021android}. 
% While these approaches provide valuable insights, they often fail to capture the nuanced and complex behaviors that characterize modern malware.
% \toolname is the fist work to enable DexBERT~\cite{sun2023dexbert} to detect Android malware with its powerful representation learning capabilities, from a novel perspective of multiple instance learning.

% The evolution of malware detection has been marked by a continuous battle against the emergence of new and sophisticated malware varieties. 
Traditional Android malware detection methods have increasingly fallen short in addressing the complexity of malware varieties~\cite{qiu2020survey,chowdhury2023android}. The integration of machine learning~\cite{arp2014drebin,wu2019malscan} and deep learning techniques~\cite{hsien2018r2,ding2020android,daoudi2021dexray} into the field represents a significant advancement, promising enhanced detection capabilities.
Nonetheless, the application of these sophisticated approaches in Android malware detection encounters substantial challenges, as they largely rely on static analysis~\cite{fereidooni2016anastasia,sandeep2019static,pan2020systematic}, low-level bytecode~\cite{daoudi2021dexray,sun2021android}, and function call graphs~\cite{pektacs2020deep,yang2021android}, potentially overlooking the intricate behaviors inherent in modern malware.
\toolname is the fist endeavor to enable DexBERT~\cite{sun2023dexbert} to detect Android malware with a comprehensive app-level representation, from a novel perspective of multiple instance learning.

% Multiple Instance Learning (MIL) has attracted increasing research interests and applications in recent years. 
% The application scenarios of MIL span across various domains~\cite{ji2020diversified,song2019using,hebbar2021deep}, but the most prominent one is Medical Imaging and Diagnosis~\cite{shao2021transmil,zhang2022dtfd}.
% Recently, it starts to play a key role in natural language processing~\cite{ji2020diversified,sun2023laficmil}, but its application in software engineering, especially Android, is under-explored.

Multiple Instance Learning (MIL) has attracted increasing research interest and has been applied in various fields~\cite{ji2020diversified,song2019using,hebbar2021deep} in recent years. While MIL is extensively applied in medical imaging and diagnosis, evidenced by significant contributions in the literature~\cite{shao2021transmil,zhang2022dtfd}, it has also begun to make substantial impacts in natural language processing~\cite{ji2020diversified,sun2023laficmil}. However, the application of MIL within software engineering, particularly in the context of Android malware detection, remains relatively under-explored. This gap presents a unique opportunity to extend the benefits of MIL's robust analytical capabilities to enhance software security measures in mobile platforms.


